What Distributions are Robust to Indiscriminate Poisoning Attacks for Linear Learners?

We study indiscriminate poisoning for linear learners where an adversary injects a few crafted examples into the training data with the goal of forcing the induced model to incur higher test error. Inspired by the observation that linear learners on some datasets are able to resist the best known attacks even without any defenses, we further investigate whether datasets can be inherently robust to indiscriminate poisoning attacks for linear learners. For theoretical Gaussian distributions, we rigorously characterize the behavior of an optimal poisoning attack, defined as the poisoning strategy that attains the maximum risk of the induced model at a given poisoning budget. Our results prove that linear learners can indeed be robust to indiscriminate poisoning if the class-wise data distributions are well-separated with low variance and the size of the constraint set containing all permissible poisoning points is also small. These findings largely explain the drastic variation in empirical attack performance of the state-of-the-art poisoning attacks on linear learners across benchmark datasets, making an important initial step towards understanding the underlying reasons some learning tasks are vulnerable to data poisoning attacks.

==> 02_related_work.tex <==

\section{Related Work}
The most relevant works to ours are indiscriminate data poisoning attacks, where the attacker goal is to develop an efficient and effective method for generating a set of poisoned data points which maximizes the test error of the induced victim model. Solving the exact bi-level optimization problem is challenging from an algorithmic perspective, thus, a typical approach is to find an approximate solution using some heuristics. In particular, one line of research adopts iterative gradient-based methods to directly maximize the surrogate loss function used by the victim~\citep{biggio2011support,mei2015using,mei2015security,koh2017understanding}, which all in essence leverages the idea of influence functions, a classical technique in robust statistics~\citep{rousseeuw2011robust}. However, a major drawback of these methods is their high computation costs required for solving the Hessian inverse problem, even with some relaxation techniques adopted to accelerate the computation.




More recently, convex optimization based methods are proposed~\citep{steinhardt2017certified,suya2021model,koh2022stronger} as a more efficient way to generate poisoned data than prior approaches, but they usually requires an additional target model. These attacks either convert the challenging bi-level optimization problem into an easier convex problem using some relaxation techniques \citep{steinhardt2017certified} or sequentially generate the poisoned data points using an online learning approach based on a target model selected in advance~\citep{suya2021model,koh2022stronger}. Although theoretical guarantees on the maximum achievable surrogate loss~\citep{steinhardt2017certified} and the asymptotic convergence of the induced victim model to the target model~\citep{suya2021model}
have been proven, their attack performances highly depend on the tightness of the convex relaxation bounds or the heuristically-selected target model. Therefore, it remains unclear whether these methods are able to generate 
(near) optimal solutions to the original bi-level optimization problem.






==> 06_theory_general.tex <==

\subsection{General Case}
\snote{The importance of this section is to link the high dimension problem and 1D case by projection, which is what we did when explaining the benchmark datasets. However, due to the space, we may optioally move this section to appendix and then talk about implications for the general case as a sentence, but prefer to keep it here}
In this section, we consider general data distributions $\mu_c$ with high-dimensional inputs. More specifically, we are going to first characterize a necessary condition for the optimal poisoning adversary $\cA_{\opt}$ defined in Definition \ref{def:optimal poisoning attack}, then discuss several inherent properties related to $\mu_c$, $\cC$ and $\eps$, which potentially cause vulnerabilities to indiscriminate poisoning attack.


According to Theorem \ref{thm:optimal ratio} and Remark \ref{rem:optimal poisoning ratio}, we know the optimal poisoning performance defined in Definition \ref{def:optimal poisoning attack} can be achieved with $\delta = \epsilon$ for linear models and hinge loss, thus we will only consider $\delta = \eps$ in the following discussions. 

To begin with, we introduce the following notations and definitions for simplicity. Consider the linear hypothesis class $\cH_{\mL}$. 
Denote the $n$-dimensional sphere by $\cS^n = \{\bw\in\RR^n: \|\bw\|_2 = 1\}$.
For any $\mu_p$ and any $\bw\in\cS^n$, $b_p^*(\bw;\mu_p)$ be the clean loss minimizer and poisoned loss minimizer conditioned on $\bw$, respectively. Namely,
\begin{align*}
    b_c^*(\bw) = \argmin_{b\in\RR}\:L(h_{\bw,b};\mu_c), \quad b_p^*(\bw; \mu_p) = \argmin_{b\in\RR}\:\big[L(h_{\bw,b};\mu_c) + \eps\cdot L(h_{\bw,b};\mu_p)\big].
\end{align*}
 Let $\mu_p^*$ be the poisoned data distribution generated by $\cA_\opt$.
Assume $h_p^* := h_{\bw_p^*, b_p*(\bw_p^*; \mu_p^*)}$ is the hypothesis induced by $\mu_p^*$:
\begin{align*}
    h_{\bw_p^*, b_p*(\bw_p^*; \mu_p^*)} = \argmin_{h_{\bw,b}\in\cH_\mL} \big[L(h_{\bw,b};\mu_c) + \eps\cdot L(h_{\bw,b};\mu_p^*)\big].
\end{align*}
According the global optimality condition of $h_p^*$, for any $\bw\in\cS^n$, we have
\begin{align*}
    L(h_p^*; \mu_c)\leq L(h_p^*; \mu_c) + \eps\cdot L(h_p^*;\mu_p^*) \leq L(h_{\bw, b_p^{*}(\bw;\mu_p^*)}; \mu_c) + \eps\cdot L(h_{\bw, b_p^{*}(\bw;\mu_p^*)}; \mu_p^*),
\end{align*}
where the first inequality holds because hinge loss is always non-negative.
Taking the minimum over $\bw$ for both sizes of the above inequality, we can further characterize an upper bound on the clean risk of $h_p^*$: 
\begin{align}
\label{eq:upper bound optimal attack}
     \nonumber \Risk(h_p^*; \mu_c) \leq L(h_p^*; \mu_c) 
     \nonumber &\leq \min_{\bw\in\cS^n}\: \bigg[L(h_{\bw, b_p^{*}(\bw;\mu_p^*)}; \mu_c) + \eps\cdot L(h_{\bw, b_p^{*}(\bw;\mu_p^*)}; \mu_p^*)\bigg] \\
    \nonumber &\leq \min_{\bw\in\cS^n}\: \bigg[L(h_{\bw, b_c^*(\bw)}; \mu_c) + \eps\cdot L(h_{\bw, b_c^*(\bw)}; \mu_p^*)\bigg]
    \\
    &\leq \eps + \min_{\bw\in\cS^n}\: \bigg[ L(h_{\bw, b_c^{*}(\bw)}; \mu_c) + \eps\cdot \max_{\bx\in\cC} \:\bw^\top\bx \bigg], 
\end{align}
where the third inequality follows from the optimality condition of $b_p^*(\bw;\mu_p^*)$ with respect to $L(h_{\bw, b}; \mu_c) + \eps\cdot L(h_{\bw, b};\mu_p^*)$ for any $\bw$, and the last inequality follows from the fact that maximum poisoned hinge loss is achieved by poisoning at most extreme locations.

\xnote{We can first get an estimate of the right hand size of \eqref{eq:upper bound optimal attack} for benchmark datasets. It essentially boils down to searching for a weight parameter $\bw$ that both separates the clean data well and incurs small $\max_{\bx\in\cC} \:\bw^\top\bx$. 
This bound is similar to the upper bound proposed in \cite{steinhardt2017certified}, but we use it in a different way.
If $\cC$ is defined by a set of axis-aligned box constraints, it is highly relevant to sparsity-induced linear classification methods, such as $\ell_1$-norm regularized SVMs.
This could be one of the properties that cause inherent vulnerability.}

\xnote{After this, we can characterize the optimal poisoning performance with respect to $\bw$ that incurs a small clean loss. Intuitively, those $\bw$'s are more likely to be feasible choices, so if the largest risk that can be achieved by moving the bias parameter to the best location (the derivative of clean loss is limited by $[-\eps, \eps]$) will also reveal some intrinsic properties. For example, if there is always a "strong resistance" to move $b$ away from $b_c^*$ (I suspect this would also be the case for MNIST 1-7), than the dataset will be intrinsically more difficult to poisoning.}



\xnote{The first inequality (risk -> loss) could be loose in some scenarios, so it would be interesting to understand the inherent properties of $\mu_c$ that control the tightness of the bound. Especially, this will be useful if the upper bound \eqref{eq:upper bound optimal attack} is indeed very loose. We can look into some properties related to $\mu_c$ like the variations of risk, loss and their ratio w.r.t. different choices of weight parameters $\bw$ and different choices of bias parameters, provided that they are feasible. Intuitively, the upper bound \eqref{eq:upper bound optimal attack} does not explain much from the perspective of risk, but clean risk is the key metric for measuring attacking performance, so I think we would very much want to incorporate risk in the discussions.}

==> 08_discussion.tex <==
\section{Conclusion}
\label{sec:discussion}
Motivated by the empirical observation that different datasets show significantly different vulnerabilities to state-of-the-art poisoning attacks, we rigorously characterize the optimal attack for Gaussian distributions and showed that the insights learned from theoretical analysis can be used to explain and predict the vulnerabilities of benchmark datasets. We made an initial but important step towards understanding the inherent dataset properties that cause vulnerability to poisoning attacks, which may provide guidance for building more robust systems through better feature transformations. One limitation of our work is that we only analyze optimal attacks for theoretical distributions, whereas an interesting future work is to characterize the behavior of optimal poisoning attacks for high-dimensional general distributions.   




